VIREL: A Variational Inference Framework for Reinforcement Learning

Applying probabilistic models to reinforcement learning (RL) enables the application of powerful optimisation tools such as variational inference to RL. However, existing inference frameworks and their algorithms pose significant challenges for learning optimal policies, e.g., the absence of mode capturing behaviour in pseudo-likelihood methods and difficulties learning deterministic policies in maximum entropy RL based approaches. We propose VIREL, a novel, theoretically grounded probabilistic inference framework for RL that utilises a parametrised action-value function to summarise future dynamics of the underlying MDP. This gives VIREL a mode-seeking form of KL divergence, the ability to learn deterministic optimal polices naturally from inference and the ability to optimise value functions and policies in separate, iterative steps. In applying variational expectation-maximisation to VIREL we thus show that the actor-critic algorithm can be reduced to expectation-maximisation, with policy improvement equivalent to an E-step and policy evaluation to an M-step. We then derive a family of actor-critic methods from VIREL, including a scheme for adaptive exploration. Finally, we demonstrate that actor-critic algorithms from this family outperform state-of-the-art methods based on soft value functions in several domains.

==> VIREL NeurIPS i/sections/abstract.tex <==
\vspace{-0.55cm}
\begin{abstract}
Applying probabilistic models to reinforcement learning (RL) enables the uses of powerful optimisation tools such as variational inference in RL. However, existing inference frameworks and their algorithms pose significant challenges for learning optimal policies, for example, the lack of mode capturing behaviour in pseudo-likelihood methods, difficulties learning deterministic policies in maximum entropy RL based approaches, and a lack of analysis when function approximators are used. We propose \textsc{virel}, a theoretically grounded inference framework for RL that utilises a parametrised action-value function to summarise future dynamics of the underlying MDP, generalising existing approaches. \textsc{virel} also benefits from a mode-seeking form of KL divergence, the ability to learn deterministic optimal polices naturally from inference, and the ability to optimise value functions and policies in separate, iterative steps. Applying variational expectation-maximisation to \textsc{virel}, we show that the actor-critic algorithm can be reduced to expectation-maximisation, with policy improvement equivalent to an E-step and policy evaluation to an M-step. We  derive a family of actor-critic methods from \textsc{virel}, including a scheme for adaptive exploration and demonstrate that our algorithms outperform state-of-the-art methods based on soft value functions in several domains.
\end{abstract}

==> VIREL NeurIPS i/sections/acknowledgements.tex <==
\section{Acknowledgements}
\vspace{-0.3 cm}
This project has received funding from the European Research Council (ERC) under the European Unions Horizon
2020 research and innovation programme (grant agreement
number 637713). The experiments were made possible by
a generous equipment grant from NVIDIA. Matthew Fellows is funded by the EPSRC. Anuj Mahajan is funded by Google DeepMind and the Drapers Scholarship. Tim G. J. Rudner is funded by the Rhodes Trust and the EPSRC. We would like to thank Yarin Gal and Piotr Miloś for helpful comments.



==> VIREL NeurIPS i/sections/actor_critic.tex <==
\vspace{-0.2cm}
\section{Actor-Critic and EM}
\vspace{-0.1cm}

\label{sec:acem}
We now apply the expectation-maximisation (EM) algorithm \citep{Dempster77maximumlikelihood,Gunawardana05} to optimise our objective $\lp$. (See \cref{sec:inference_background} for an exposition of this algorithm.) In keeping with RL nomenclature, we refer to $\hQ$ as the \emph{critic} and $\pit$ as the \emph{actor}. We establish that the expectation (E-) step is equivalent to carrying out policy improvement and the maximisation (M-)step to policy evaluation. This formulation reverses the situation in most pseudo-likelihood methods, where the E-step is related to policy evaluation and the M-step is related to policy improvement, and is a direct result of optimising the forward KL divergence, $\kl{q_\theta(h)}{\pw(h\vert \mathcal{O})}$, as opposed to the reverse KL divergence used in pseudo-likelihood methods. As discussed in \cref{sec:PL}, this mode-seeking objective prevents the algorithm from learning risk-seeking policies.
We now introduce an extension to \cref{assumption:policy_represent_optimal} that is sufficient to guarantee convergence.

\begin{assumption}[Universal Variational Representability]\label{assumption:policy_represent}
Every Boltzmann policy can be represented as $\pi_\theta(a\vert s)$, i.e., $\forall\ \omega\in\Omega\ \exists\ \theta\in\Theta\ s.t.\ \pit=\piw$.
\end{assumption}
\cref{assumption:policy_represent} is strong but, like in variational inference, our variational policy $\pi_\theta(a\vert s)$ provides a useful approximation when \cref{assumption:policy_represent} does not hold. As we discuss in \cref{sec:relaxation_assumption}, using projected Bellman errors also ensures that our M-step always converges no matter what our current policy is.

\vspace{-0.3cm}
\subsection{Variational Actor-Critic}
\vspace{-0.1cm}
\label{sec:vacem}
In the E-step, we keep the parameters of our critic $\omega_k$ constant while updating the actor's parameters by maximising the ELBO with respect to $\theta$: $\theta_{k+1}\leftarrow \argmax_\theta\mathcal{L}(\omega_k,\theta)$. Using gradient ascent with step size $\alpha_{\textrm{actor}}$, we optimise $\varepsilon_{\omega_k}\mathcal{L}(\omega_k,\theta)$ instead, which prevents ill-conditioning and does not alter the optimal solution, yielding the update (see \cref{proof:estep} for full derivation):
\vspace{-0.2cm}
\paragraph{ E-Step (Actor):} $\theta_{i+1}\leftarrow\theta_{i} + \alpha_{\textrm{actor}}\left(\varepsilon_{\omega_k}\nabla_\theta \mathcal{L}(\omega_k,\theta)\right)\rvert_{\theta=\theta_i}$,\\
\vspace{-0.2cm}
\begin{align}
\varepsilon_{\omega_k}\nabla_\theta \mathcal{L}(\omega_k,\theta)=\mathbb{E}_{s\sim d(s)}\left[\mathbb{E}_{a\sim\pit}\left[ \hat{Q}_{\omega_k}(h)\nabla_\theta\log\pit\right]+\varepsilon_{\omega_k}\nabla_\theta\mathscr{H}(\pit)\right].\label{eq:e_step}
\end{align}
In the M-step, we maximise the ELBO with respect to $\omega$ while holding the parameters $\theta_{k+1}$ constant. Hence expectations are taken with respect to the variational policy found in the E-step: $\omega_{k+1}\leftarrow \argmax_\omega\mathcal{L}(\omega,\theta_{k+1})$. We use gradient ascent with step size $\alpha_\textrm{critic}(\varepsilon_{\omega_i})^2$ to optimise $\mathcal{L}(\omega,\theta_{k+1})$ to prevent ill-conditioning, yielding (see \cref{proof:mstep} for full derivation):
\paragraph{M-Step (Critic):} $
\omega_{i+1}\leftarrow\omega_{i} + \alpha_{\textrm{critic}}(\varepsilon_{\omega_i})^2\nabla_\omega \mathcal{L}(\omega,\theta_{k+1})\rvert_{\omega=\omega_i},$
\begin{align}
&(\varepsilon_{\omega_i})^2\nabla_\omega \mathcal{L}(\omega,\theta_{k+1})=\varepsilon_{\omega_i}\mathbb{E}_{ d(s)\pi_{\theta_{k+1}}(a\vert s)}\left[ \nabla_\omega\hQ\right]-\mathbb{E}_{ d(s)\pi_{\theta_{k+1}}(a\vert s)}\left[ \hat{Q}_{\omega_i}(h)\right]\nabla_\omega\ew.\label{eq:m_step}
\end{align}
\vspace{-0.6cm}
\subsection{Discussion}
\label{sec:ac_discuss}
From an RL perspective, the E-step corresponds to training an actor using a policy gradient method \citep{Sutton00} with an adaptive entropy regularisation term \citep{Williams91,Mnih16}. The M-step update corresponds to a policy evaluation step, as we seek to reduce the MSBE in the second term of \cref{eq:m_step}. We derive $\nabla_\omega\ew$ exactly in \cref{sec:gradient_residual_error}. Note that this term depends on $(\tw\hQ-\hQ)\nabla_\omega\tw\hQ$, which typically requires evaluating two independent expectations. For convergence guarantees, techniques such as residual gradients \citep{Baird95} or GTD2/TDC \citep{Maei09} need to be employed to obtain an unbiased estimate of this term. If guaranteed convergence is not a priority, dropping gradient terms allows us to use direct methods \citep{Sutton17}, which are often simpler to implement. We discuss these methods further in \cref{sec:approx_gradients} and provide an analysis in \cref{sec:analysis_of_approximations} demonstrating that the corresponding updates act as a variational approximation to $Q$-learning \citep{qlearning,dqn}. A key component of our algorithm is the behaviour when $\varepsilon_{\omega^*}=0$; under this condition, there is no M-step update (both $\varepsilon_{\omega_k}=0$ and $\nabla_\omega\ew=0$) and $Q_{\omega^*}(h)=Q^*(h)$ (see \cref{proof:forward}), so our E-step reduces exactly to a policy gradient step, $\theta_{k+1}\leftarrow\theta_{k} + \alpha_{\textrm{actor}}\mathbb{E}_{h\sim d(s)\pit}\left[ Q^*(h)\nabla_\theta\log\pit\right]$, recovering the optimal policy in the limit of convergence, that is, $\pit\rightarrow\pi^*(a\vert s)$.

From an inference perspective, the E-step improves the parameters of our variational distribution to reduce the gap between the current Boltzmann posterior and the variational policy, $\kl{\pit)}{\pi_{\omega_k}(a\vert s)}$ (see \cref{proof:policy_posterior}). This interpretation makes precise the intuition that how much we can improve our policy is determined by how similar $\hat{Q}_{\omega_k}(h)$ is to $Q^*(h)$, limiting policy improvement to the complete E-step:
$\pi_{\theta_{k+1}}(a\vert s)=\pi_{\omega_k}(a\vert s)$. We see that the common greedy policy improvement step, $\pi_{\theta_{k+1}}(a\vert s)=\delta(a\in\argmax_{a'}(\hat{Q}_{\omega_k}(a',s)))$ acts as an approximation to the Boltzmann form in \cref{eq:action_posterior}, replacing the softmax with a hard maximum.

If \cref{assumption:policy_represent} holds and any constraint induced by $\tw\boldsymbol{\cdot}$ does not prevent convergence to a complete E-step, the EM algorithm alternates between two convex optimisation schemes, and is guaranteed to converge to at least a local optimum of $\mathcal{L}(\omega,\theta)$ \citep{Wu83}. In reality, we cannot carry out complete E- and M-steps for complex domains, and our variational distributions are unlikely to satisfy \cref{assumption:policy_represent}. Under these conditions, we can resort to the empirically successful variational EM algorithm \citep{Jordan1999}, carrying out partial E- and M-steps instead, which we discuss further in \cref{sec:approx_gradients}.

\subsection{Advanced Actor-Critic Methods}
\label{sec:relationship_to_pg}
A family of actor-critic algorithms follows naturally from our framework: 1) we can use powerful inference techniques such as control variates \citep{qprop} or variance-reducing baselines by subtracting any function that does not depend on the action \citep{Schulman15a}, e.g., $V(s)$, from the action-value function, as this does not change our objective, 2) we can manipulate \cref{eq:e_step} to obtain variance-reducing gradient estimators such as EPG \citep{epg-journal}, FPG \citep{fpg}, and SVG0 \citep{Heess15}, and 3) we can take advantage of $d(s)$ being any general decorrelated distribution by using replay buffers \citep{dqn} or empirically successful asynchronous methods that combine several agents' individual gradient updates at once \citep{Mnih16}. As we discuss in \cref{sec:E-step_discussion}, the manipulation required to derive the estimators in 2) is not strictly justified in the classic policy gradient theorem \citep{Sutton00} and MERL formulation \citep{Haarnoja18}.

MPO is a state-of-the-art EM algorithm derived from the pseudo-likelihood objective \citep{Abdolmaleki18}. In its derivation, policy evaluation does not naturally arise from either of its EM steps and must be carried out separately. In addition, its E step is approximated, giving rise to the one step KL regularised update. As we demonstrate in \cref{sec:recovering_mpo}, under the probabilistic interpretation of our model, including a prior of the form $p_\phi(h)=\mathcal{U}(s)\pip$ in our ELBO and specifying a hyper-prior $p(\omega)$, the MPO objective with an adaptive regularisation constant can be recovered from \textsc{virel}: 
\begin{align}
\mathcal{L}^\textsc{mpo}(\omega,\theta,\phi)=\mathbb{E}_{s\sim d(s)}\left[\mathbb{E}_{a\sim \pit}\left[ \frac{\hQ}{\ew}\right]-\kl{\pit}{\pip }\right]+\log p(\omega).
\end{align}
We also show in \cref{sec:recovering_mpo} that applying the (variational) EM algorithm from \cref{sec:acem} yields the MPO updates with the missing policy evaluation step and without approximation in the E-step.


==> VIREL NeurIPS i/sections/background.tex <==
\section{Background}
\label{sec:background}

We assume familiarity with probabilistic inference \citep{Jordan1999} and provide a review in \cref{sec:inference_background}.

\subsection{Reinforcement Learning}
\label{sec:rl_objective}

Formally, an RL problem is modelled as a Markov decision process (MDP) defined by the tuple $\langle \mathcal{S},\mathcal{A},r,p,p_0,\gamma \rangle$ \citep{sutton, rl_algorithms}, where $\mathcal{S}$ is the set of states and $\mathcal{A}\subseteq \mathbb{R}^n$ the set of available actions.
An agent in state $s\in\mathcal{S}$ chooses an action $a\in\mathcal{A}$ according to the policy $a\sim\pi(\cdot\vert s)$, forming a state-action pair $h\in\mathcal{H}$, $h\coloneqq\langle s,a\rangle$.
This pair induces a scalar reward according to the reward function $r_t\coloneqq r(h_t)\in\mathbb{R}$ and the agent transitions to a new state $s'\sim p(\cdot\vert h)$.
The initial state distribution for the agent is given by $s_0\sim p_0$.
We denote a sampled state-action pair at timestep $t$ as $h_t\coloneqq\langle s_t,a_t\rangle$.
As the agent interacts with the environment using $\pi$, it gathers a trajectory $\tau=(h_0,r_0,h_1,r_1,...)$. The value function is the expected, discounted reward for a trajectory, starting in state $s$. The action-value function or $Q$-function is the expected, discounted reward for each trajectory, starting in $h$, $
Q^\pi(h)\coloneqq \mathbb{E}_{\tau\sim p^\pi(\tau\vert h)}\left[\sum_{t=0}^{\infty}\gamma^tr_t\right]$, where $p^\pi(\tau\vert h)\coloneqq p(s_1\vert h_0=h)\prod_{t'=1}^{\infty}p(s_{t'+1}\vert h_{t'})\pi(a_t\vert s_t)$. Any $Q$-function satisfies a Bellman equation $\mathcal{T}^\pi Q^\pi(\cdot)=Q^\pi(\cdot)$ where $\mathcal{T}^\pi\boldsymbol{\cdot}\coloneqq r(h)+\gamma \mathbb{E}_{h'\sim p(s'\vert h)\pi(a'\vert s')}\left[\boldsymbol{\cdot}\right]$ is the Bellman operator. We consider infinite horizon problems with a discount factor $\gamma\in[0,1)$.
The agent seeks an optimal policy $\pi^{*} \in \argmax_{\pi}{J^\pi}$, where
\begin{align}
J^\pi=\mathbb{E}_{h\sim p_0(s)\pi(a\vert s)}\left[ Q^\pi(h)\right]. \label{eq:rl_objective} 
\end{align}
We denote optimal $Q$-functions as $Q^*(\cdot)\coloneqq Q^{\pi^*}(\cdot)$ and the set of optimal policies $\Pi^*\coloneqq\argmax_{\pi}{J^\pi}$. The optimal Bellman operator is $\mathcal{T}^*\boldsymbol{\cdot}\coloneqq r(h)+\gamma \mathbb{E}_{h'\sim p(s'\vert h)}\left[\max_{a'}(\boldsymbol{\cdot})\right]$.


\subsection{Maximum Entropy RL}
\label{sec:MERL}
The MERL objective supplements each reward in the RL objective with an entropy term \citep{Todorov06, Ziebart08,Ziebart10a, Ziebart10b}, $J_{\textrm{merl}}^\pi\coloneqq\mathbb{E}_{\tau\sim p(\tau)}\left[\sum_{t=0}^{T-1}\left( r_t-c\log(\pi (a_t\vert s_t)\right)\right]$. The standard RL, undiscounted objective is recovered for $c\rightarrow0$ and we assume $c=1$ without loss of generality. The MERL objective is often used to motivate the MERL inference framework (which we call \textsc{merlin}) \citep{Levine14}, mapping the problem of finding the optimal policy, $\pi_{\mathrm{merl}}^*(a\vert s)=\argmax_\pi J^\pi_{\textrm{merl}}$, to an equivalent inference problem. A full exposition of this framework is given by \citet{virl_review} and we discuss the graphical model of $\textsc{merlin}$ in comparison to $\textsc{virel}$ in \cref{sec:comparing_virel_merlin}. The inference problem is often solved using a message passing algorithm, where the log backward messages are called soft value functions due to their similarity to classic (hard) value functions \citep{Toussaint09b, Rawlik12, Haarnoja18, Haarnoja17,virl_review}. The soft $Q$-function is defined as
$Q_{\mathrm{soft}}^\pi(h)\coloneqq\mathbb{E}_{\tau\sim q^\pi(\tau\vert h)}\left[ r_0+\sum_{t=1}^{T-1}(r_t-\log \pi(a_t\vert s_t))\right]$,
where $q^\pi(\tau\vert h)\coloneqq p(s_0\vert h)\prod_{t=0}^{T-1}p(s_{t+1}\vert h_t)\pi(a_t\vert s_t)$. The corresponding soft Bellman operator is $\mathcal{T}^{\pi}_{\mathrm{soft}}\boldsymbol{\cdot}\coloneqq r(h)+\mathbb{E}_{h'\sim p(s'\vert h)\pi(a'\vert s')}[\boldsymbol{\cdot}-\log\pi(a'\vert s')]$. Several algorithms have been developed that mirror existing RL algorithms using soft Bellman equations, including maximum entropy policy gradients \citep{virl_review}, soft $Q$-learning \citep{Haarnoja17}, and soft actor-critic (SAC) \citep{Haarnoja18}. MERL is also compatible with methods that use recall traces \citep{Goyal18}. 
 \begin{wrapfigure}{l}{0.45\textwidth}
	\centering
	\vspace{-0.2cm}
		\includegraphics[width=0.45\columnwidth]{counterexample.pdf}
	\caption{A discrete MDP counterexample for optimal policy under maximum entropy.}
	\label{ce}
	\vspace{-0.5cm}
\end{wrapfigure}

We now outline key drawbacks of \textsc{merlin}. It is well-understood that optimal policies under regularised Bellman operators are more stochastic than under their equivalent unregularised operators \citep{geist19a}. While this can lead to improved exploration, the optimal policy under these operators will still be stochastic, meaning optimal deterministic policies are not learnt naturally. This leads to two difficulties: 1) a deterministic policy can be constructed by taking the action $a^*=\argmax_{a}\pi^*_{\textrm{merl}}(a\vert s)$, corresponding to the maximum a posteriori (MAP) policy, however, in continuous domains, finding the MAP policy requires optimising the $Q$-function approximator for actions, which is often a deep neural network. A common approximation is to use the mean of a variational policy instead; 2) even if we obtain a good approximation, as we show below by way of counterexample, the deterministic MAP policy is not guaranteed to be the optimal policy under $J^\pi$. Constraining the variational policies to the set of Dirac-delta distributions does not solve this problem either, since it renders the inference procedure intractable \citep{Rawlik10,Rawlik12}.

Next, we demonstrate that the optimal policy under $J^{\pi}$ cannot always be recovered from the MAP policy under $J^{\pi}_\textrm{merl}$. Consider the discrete state MDP as shown in \cref{ce}, with action set $\mathcal{A}=\{a_1,a_2,a_1^1,\cdots a_1^{k_1}\}$ and state set $\mathcal{S}=\{s_0,s_1,s_2,s_3,s_4,s_1^1\cdots s_1^{k_1},s_5,\cdots s_{5+{k_2}} \}$. All state transitions are deterministic, with $p(s_1\vert s_0, a_1)=p(s_1\vert s_0, a_2)=p(s_1^i\vert s_1, a_1^i)=1$. All other state transitions are deterministic and independent of action taken, that is, $p(s_j\vert \cdot, s_{j-1})=1\ \forall\ {j>2}$ and $p(s_5\vert \cdot, s_1^{i})=1$. The reward function is $r(s_0,a_2) = 1$ and zero otherwise. Clearly the optimal policy under $J^\pi$ has $\pi^*(a_2|s_0) = 1$. Define a maximum entropy reinforcement learning policy as $\pi_{\textrm{merl}}$ with  $\pi_{\textrm{merl}}(a_1|s_0)=p_1$, $\pi_{\textrm{merl}}(a_2|s_0)=(1-p_1)$ and $\pi_{\textrm{merl}}(a_1^i|s_1)=p_1^i$. For $\pi_{\textrm{merl}}$ and $k_2>>5$, we can evaluate $J^\pi_\textrm{merl}$ for any scaling constant $c$ and discount factor $\gamma$ as:
\begin{align}
    J^\pi_\textrm{merl}=(1-p_1)(1-c\log(1-p_1))-p_1\left(c\log p_1 +\gamma c\sum_{i=1}^k p_1^i \log p_1^i\right). \label{eq:counter_objective}
\end{align}
We now find the optimal MERL policy. Note that  $p_1^i=\frac{1}{k}$ maximises the final term in \cref{eq:counter_objective}. Substituting for $p_1^i=\frac{1}{k_1}$, then taking derivatives of \cref{eq:counter_objective} with respect to $p_1$, and setting to zero, we find $p_1^*=\pi_{\textrm{merl}}^*(a_1\vert s_0)$ as:
\begin{align}
    1-c\log(1-p_1^*)&=\gamma c\log(k_1)-c\log p_1^*,\\
    \implies p_1^*&=\frac{1}{{k_1}^{-\gamma}\exp\left(\frac{1}{c}\right)+1},
\end{align}
hence, for any ${k_1}^{-\gamma}\exp\left(\frac{1}{c}\right) < 1$, we have $ p_1^*>\frac{1}{2}$ and so $\pi^*$ cannot be recovered from $\pi_{\textrm{merl}}^*$, even using the mode action $a_1=\argmax_a\pi_{\textrm{merl}}^*(a\vert s_0)$. The degree to which the MAP policy varies from the optimal unregularised policy depends on both the value of $c$ and $k_1$, the later controlling the number of states with sub-optimal reward. Our counterexample illustrates that when there are large regions of the state-space with sub-optimal reward, the temperature must be comparatively small to compensate, hence algorithms derived from \textsc{merlin} become very sensitive to temperature. As we discuss in \cref{sec:comparing_virel_merlin}, this problem stems from the fact that \textsc{merl} policies optimise for expected reward and long-term expected entropy. While initially beneficial for exploration, this can lead to sub-optimal polices being learnt in complex domains as there is often too little a priori knowledge about the MDP to make it possible to choose an appropriate value or schedule for $c$. 

Finally, a minor issue with \textsc{merlin} is that many existing models are defined for finite-horizon problems \citep{virl_review, Rawlik12}. While it is possible to discount and extend \textsc{merlin} to infinite-horizon problems, doing so is often nontrivial and can alter the objective \citep{Thomas14, Haarnoja18}.
\vspace{-0.2cm}
\subsection{Pseudo-Likelihood Methods}
\vspace{-0.1cm}
\label{sec:PL}

A related but distinct approach is to apply Jensen's inequality directly to the RL objective $J^\pi$. Firstly, we rewrite \cref{eq:rl_objective} as an expectation over $\tau$ to obtain $J=\mathbb{E}_{h\sim p_0(s)\pi(a\vert s)}\left[ Q^\pi(h)\right]=\mathbb{E}_{\tau\sim p(\tau)}\left[ R(\tau) \right]$, where $R(\tau)=\sum_{t=0}^{T-1}\gamma^tr_t$ and $p(\tau)=p_0(s_0)\pi(a_0\vert s_o)\prod^{T-1}_{t=0}p(h_{t+1}\vert h_{t})$. We then treat $p(R,\tau)=R(\tau)p(\tau)$ as a joint distribution, and if rewards are positive and bounded, Jensen's inequality can be applied, enabling the derivation of an evidence lower bound (ELBO). Inference algorithms such as EM can then be employed to find a policy that optimises the pseudo-likelihood objective \citep{Dayan97, Toussaint06b,Peters07,Hachiya09,Neumann11,Abdolmaleki18}. Pseudo-likelihood methods can also be extended to a model-based setting by defining a prior over the environment's transition dynamics. \citet{Furmston2010} demonstrate that the posterior over all possible environment models can be integrated over to obtain an optimal policy in a Bayesian setting. 

Many pseudo-likelihood methods minimise $\kl{p_{\mathcal{O}}}{p_{\pi}}$, where $p_{\pi}$ is the policy to be learnt and $p_{\mathcal{O}}$ is a target distribution monotonically related to reward \citep{virl_review}. Classical RL methods minimise $\kl{p_{\pi}}{p_{\mathcal{O}}}$. The latter encourages learning a mode of the target distribution, while the former encourages matching the moments of the target distribution. If the optimal policy can be represented accurately in the class of policy distributions, optimisation converges to a global optimum and the problem is fully observable, the optimal policy is the same in both cases. Otherwise, the  pseudo-likelihood objective reduces the influence of large negative rewards, encouraging risk-seeking policies.


==> VIREL NeurIPS i/sections/conclusion.tex <==
\vspace{-0.1cm}
\section{Conclusion and Future Work}
\vspace{-0.2cm}
\label{sec:conclusion}
This paper presented \textsc{virel}, a novel framework that recasts the reinforcement learning problem as an inference problem using function approximators. We provided strong theoretical justifications for this framework and compared two simple actor-critic algorithms that arise naturally from applying variational EM on the objective. Extensive empirical evaluation shows that our algorithms perform on par with current state-of-the-art methods on simple domains and substantially outperform them on challenging high dimensional domains. As immediate future work, our focus is to find better estimates of $\ew$ to provide a principled method for uncertainty based exploration; we expect it to help attain sample efficiency in conjunction with various methods like \citep{mahajan2017asymmetry,mahajan2017symmetry}. Another avenue of research would extend our framework to multi-agent settings, in which it can be used to tackle the sub-optimality induced by representational constraints used in MARL algorithms \citep{mahajan2019maven}.

==> VIREL NeurIPS i/sections/experiments.tex <==
\vspace{-0.5cm}
\section{Experiments}
\vspace{-0.1cm}
\label{sec:experiments}
%PLOTS
We evaluate our EM algorithm using the direct method approximation outlined in \cref{sec:approx_gradients} with $\tw$, ignoring constraints on $\Omega$. The aim of our evaluation is threefold: Firstly, as explained in \cref{sec:model}, algorithms using soft value functions cannot be recovered from \textsc{virel}. We therefore demonstrate that using hard value functions does not affect performance. Secondly, we provide evidence for our hypothesis stated in \cref{sec:comparing_virel_merlin} that using soft value functions may harm performance in higher dimensional tasks. Thirdly, we show that even under all practical approximations discussed, the algorithm derived in \cref{sec:acem} still outperforms advanced actor-critic methods.

We compare our methods to the state-of-the-art SAC\footnote{We use implementations provided by the authors \url{https://github.com/haarnoja/sac} for v1 and \url{https://github.com/vitchyr/rlkit} for v2.} and DDPG \citep{lillicrap2015continuous}  algorithms on MuJoCo tasks in OpenAI gym \citep{openai} and in rllab~\citep{rllab}. We use SAC as a baseline because \citet{Haarnoja18} show that it outperforms PPO \citep{Schulman2017ppo}, Soft $Q$-Learning \citep{Haarnoja17}, and TD3 \citep{fujimoto2018addressing}. We compare to DDPG \citep{lillicrap2015continuous}  because, like our methods, it can learn deterministic optimal policies. We consider two variants: In the first one, called \textit{virel}, we keep the scale of the entropy term in the gradient update for the variational policy constant $\alpha$; in the second, called \textit{beta}, we use an estimate $\he$ of $\ew$ to scale the corresponding term in \cref{eq:E-step_full}. We compute $\he$ using a buffer to draw a fixed number of samples $N_{\varepsilon}$ for the estimate. 
\begin{figure*}[!htb]
\vspace{-0.4cm}
	\begin{center}
		\minipage{0.33\textwidth}
		\includegraphics[width=\linewidth]{final_Ant-v2.pdf}
		\label{fig:antv2}
		\endminipage
		\minipage{0.33\textwidth}
		\includegraphics[width=\linewidth]{final_Humanoid-v2.pdf}
		\label{fig:humanoidv2}
		\endminipage
		\minipage{0.33\textwidth}
		\includegraphics[width=\linewidth]{final_HumanoidStandup-v2.pdf}
		\label{fig:reacherv2}
		\endminipage\\
	\end{center}
\vspace{-5mm}
	\caption{Training curves on continuous control benchmarks gym-Mujoco-v2 : High-dimensional domains.}
		\vspace{-5mm}
	\label{experimentsv2}
\end{figure*}

To adjust for the relative magnitude of the first term in \cref{eq:E-step_full} with that of $\ew$ scaling the second term, we also multiply the estimate $\he$ by a scalar $\lambda\approx \frac{1-\gamma}{r_{avg}}$, where $r_{avg}$ is the average reward observed; $\lambda^{-1}$ roughly captures the order of magnitude of the first term and allows $\he$ to balance policy changes between exploration and exploitation. We found performance is poor and unstable without $\lambda$. To reduce variance, all algorithms use a value function network $V(\phi)$ as a baseline and a Gaussian policy, which enables the use of the reparametrisation trick. Pseudocode can be found in \cref{app:pseudocode}. All experiments use 5 random initialisations and parameter values are given in \cref{paremeter_values}.


\cref{experimentsv2} gives the training curves for the various algorithms on high-dimensional tasks for on gym-mujoco-v2. In particular, in Humanoid-v2 (action space dimensionality: 17, state space dimensionality: 376) and Ant-v2 (action space dimensionality: 8, state space dimensionality: 111), DDPG fails to learn any reasonable policy.  We believe that this is because the Ornstein-Uhlenbeck noise that DDPG uses for exploration is insufficiently adaptive in high dimensions. While SAC performs better, \textit{virel} and \textit{beta} still significantly outperform it. As hypothesised in \cref{sec:comparing_virel_merlin}, we believe that this performance advantage arises because the gap between optimal unregularised policies and optimal variational policies learnt under \textsc{merlin} is sensitive to temperature $c$. This effect is exacerbated in high dimensions where there may be large regions of the state-action space with sub-optimal reward. All algorithms learn optimal policies in simple domains, the training curves for which can be found  in \cref{experimentsv2_app} in \cref{sec:v2_experiments}. Thus, as the state-action dimensionality increases, algorithms derived from \textsc{virel} outperform SAC and DDPG.

\citet{fujimoto2018addressing} and \citet{doubleq} note that using the minimum of two randomly initialised action-value functions helps mitigate the positive bias introduced by function approximation in policy gradient methods. Therefore, a variant of SAC uses two soft critics.  We compare this variant of SAC to two variants of \textit{virel}: \textit{virel1}, which uses two hard $Q$-functions and \textit{virel2}, which uses one hard and one soft $Q$-function. We scale the rewards so that the means of the $Q$-function estimates in \textit{virel2} are approximately aligned. \cref{experiments} shows the training curves on three gym-Mujoco-v1 domains, with additional plots shown in \cref{experimentsv1_app} in \cref{sec:v1_experiments}. Again, the results demonstrate that \textit{virel1} and \textit{virel2} perform on par with SAC in simple domains like Half-Cheetah and outperform it in challenging high-dimensional domains like humanoid-gym and -rllab (17 and 21 dimensional action spaces, 376 dimensional state space). 

\begin{figure*}[!htb]
\vspace{-0.3cm}
\begin{center}
\minipage{0.33\textwidth}
  \includegraphics[width=\linewidth]{humanoid-rllab50.pdf}
  \label{fig:swimmer}
\endminipage
\minipage{0.33\textwidth}
  \includegraphics[width=\linewidth]{humanoid50.pdf}
  \label{fig:humanoid}
\endminipage
\minipage{0.33\textwidth}
  \includegraphics[width=\linewidth]{halfc50.pdf}
  \label{fig:walker}
\endminipage
\end{center}
\vspace{-0.5cm}
\caption{Training curves on continuous control benchmarks gym-Mujoco-v1.}
\vspace{-0.5cm}
\label{experiments}
\end{figure*}

==> VIREL NeurIPS i/sections/introduction.tex <==
\vspace{-0.3cm}
\section{Introduction}
\label{sec:introduction}
\vspace{-0.1cm}
Efforts to combine reinforcement learning (RL) and probabilistic inference have a long history, spanning diverse fields such as control, robotics, and RL \citep{Toussaint06b,Toussaint09a,Peters07,Rawlik10,Heess12,Ziebart08,Ziebart10a,Ziebart10b,Levine13}. Formalising RL as probabilistic inference enables the application of many approximate inference tools to reinforcement learning, extending models in flexible and powerful ways \citep{virl_review}. 
However, existing methods at the intersection of RL and inference suffer from several deficiencies.  Methods that derive from the pseudo-likelihood inference framework \citep{Dayan97, Toussaint06b, Peters07, Hachiya09, Neumann11, Abdolmaleki18} and use expectation-maximisation (EM)  favour risk-seeking policies \citep{Levine14}, which can be suboptimal. Yet another approach, the MERL inference framework \citep{virl_review} (which we refer to as \textsc{merlin}), derives from maximum entropy reinforcement learning (MERL) \citep{Koller00, Ziebart08,Ziebart10a,Ziebart10b}. While \textsc{merlin} does not suffer from the issues of the pseudo-likelihood inference framework, it presents different practical difficulties. These methods do not naturally learn deterministic optimal policies and  constraining the variational policies to be deterministic renders inference intractable \citep{Rawlik10}. As we show by way of counterexample in \cref{sec:MERL}, an optimal policy under the reinforcement learning objective is not guaranteed from the optimal MERL objective. Moreover, these methods rely on soft value functions which are sensitive to a pre-defined temperature hyperparameter. 

Additionally, no existing framework formally accounts for replacing exact value functions with function approximators in the objective; learning function approximators is carried out independently of the inference problem and no analysis of convergence is given for the corresponding algorithms. 

This paper addresses these deficiencies. We introduce \textsc{virel}, an inference framework that translates the problem of finding an optimal policy into an inference problem. Given this framework, we demonstrate that applying EM induces a family of actor-critic algorithms, where the E-step corresponds exactly to policy improvement and the M-step exactly to policy evaluation. Using a variational EM algorithm, we derive analytic updates for both the model and variational policy parameters, giving a unified approach to learning parametrised value functions and optimal policies.

We extensively evaluate two algorithms derived from our framework against DDPG \citep{lillicrap2015continuous} and an existing state-of-the-art actor-critic algorithm, soft actor-critic (SAC) \cite{Haarnoja18}, on a variety of OpenAI gym domains \citep{openai}. While our algorithms perform similarly to SAC and DDPG on simple low dimensional tasks, they outperform them substantially on complex, high dimensional tasks.

The main contributions of this work are: 1) an exact reduction of entropy regularised RL to probabilistic inference using value function estimators; 
2) the introduction of a theoretically justified general framework for developing inference-style algorithms for RL that incorporate the uncertainty in the optimality of the action-value function, $\hQ$, to drive exploration, but that can also learn optimal deterministic policies; and
3) a family of practical algorithms arising from our framework that adaptively balances exploration-driving entropy with the RL objective and outperforms the current state-of-the-art SAC, reconciling existing advanced actor critic methods like A3C \cite{Mnih16}, MPO \citep{Abdolmaleki18} and EPG \cite{epg} into a broader theoretical approach. 


==> VIREL NeurIPS i/sections/model.tex <==
\vspace{-0.6cm}
\section{\textsc{virel}}
\vspace{-0.2cm}
\label{sec:rl_as_inference}
Before describing our framework, we state some relevant assumptions.
\begin{assumption}[Strictly Positive Optimal $Q$-function]\label{assumption:positive}
The optimal action-value function has a compact domain $\mathcal{H}$ and is finite and strictly positive, i.e., $0<Q^*(h)<\infty\  \forall\ h\in\mathcal{H}$. 
\end{assumption}
\vspace{-0.2cm}
MDPs for which rewards are lower bounded and finite, that is, $R\subset[r_\mathrm{min},\infty)$, satisfy the second condition of \cref{assumption:positive}; we can construct a new MDP by adding $r_\mathrm{min}$ to the reward function, ensuring that all rewards are positive and hence the optimal $Q$-function for the reinforcement learning problem is finite and strictly positive. This does not affect the optimal solution.  Now we introduce a function approximator $\hQ\approx Q^\pi(h)$ in the bounded function space $\hQ\in\mathcal{Q}_\Omega$:
\begin{definition}[Bounded Function Space] Let $\mathcal{Q}_\Omega\coloneqq\left\{f:\Omega\times\mathcal{H}\rightarrow\mathbb{R}\ \Big\vert\ \lvert f\rvert <\infty\ \forall\  \omega\in\Omega,h\in\mathcal{H} \right\}$ be the space of bounded, Lipschitz continuous functions parametrised by $\omega\in\Omega$.
\end{definition}
\begin{assumption}[Representabilty Under Optimisation]\label{assumption:policy_represent_optimal}
Our function approximator can represent the optimal $Q$-function, i.e., $\exists\ \omega^*\in\Omega\ s.t.\ Q^*(\cdot)=\hat{Q}_{\omega^*}(\cdot)$. 
\end{assumption}
\vspace{-0.2cm}
In \cref{sec:relaxation_assumption}, we extend the work of \citet{Maei09} to continuous domains, demonstrating that \cref{assumption:policy_represent_optimal} can be neglected if projected Bellman operators are used. 

\begin{assumption}[Local Smoothness of $Q$-functions ]\label{assumption:smoothness} For $\omega^*$ parametrising $Q^*(\cdot)$ in \cref{assumption:policy_represent_optimal}, $\hat{Q}_{\omega^*}(\cdot)$ has a unique maximum $\hat{Q}_{\omega^*}(h^*)=\sup_h \hat{Q}_{\omega^*}(h)$. $\hat{Q}_{\omega^*}(\cdot)$ is locally $\mathbb{C}^2$-smooth about $h^*$, i.e. $\exists\ \Delta>0\ s.t.\ \hat{Q}_{\omega^*}(h)\in\mathbb{C}^2\ \forall\ h\in\{h\vert \lVert h-h^*\rVert<\Delta$ \}.
\end{assumption}
\vspace{-0.2cm}
This assumption is formally required for the strict convergence of a Boltzmann to a Dirac-delta distribution and, as we discuss in \cref{sec:approx_local_smoothness}, is of more mathematical than practical concern. 
\vspace{-0.3cm}
\subsection{Objective Specification}
\vspace{-0.1cm}
\label{sec:model}
 We now define an objective that we motivate by satisfying three desiderata: \circled{1} In the limit of maximising our objective, a deterministic optimal policy can be recovered and the optimal Bellman equation is satisfied by our function approximator; \circled{2} when our objective is not maximised, stochastic policies can be recovered that encourage effective exploration of the state-action space; and \circled{3} our objective permits the application of powerful and tractable optimisation algorithms from variational inference that optimise the risk-neutral form of KL divergence, $\kl{p_{\pi}}{p_{\mathcal{O}}}$, introduced in \cref{sec:PL}. 
 
 Firstly, we define the residual error $\ew\coloneqq \frac{c}{p}\lVert\tw\hQ-\hQ\rVert_p^p$ where $\tw=\mathcal{T}^{\pi_\omega}\boldsymbol{\cdot}\coloneqq r(h)+\gamma \mathbb{E}_{h'\sim p(s'\vert h)\pi_\omega(a'\vert s')}\left[\boldsymbol{\cdot}\right]$ is the Bellman operator for the Boltzmann policy with temperature $\ew$:
 \begin{align}
\piw \coloneqq \frac{\exp\left(\frac{\hQ}{\ew}\right)}{\int_\mathcal{A} \exp\left(\frac{\hQ}{\ew}\right)da},\label{eq:action_posterior}
\end{align}  
where $c>0$ is an arbitrary finite constant and we assume $p=2$ and without loss of generality. Our main result in \cref{proof:forward} proves that finding a $\omega^*$ that reduces the residual error to zero, i.e., $\varepsilon_{\omega^*}=0$, is a sufficient condition for learning an optimal $Q$-function $\hat{Q}_{\omega^*}(h)=Q^*(h)$. Additionally, the Boltzmann distribution $\piw$ tends towards a Dirac-delta distribution $\piw=\delta(a=\argmax_a' \hat{Q}_{\omega^*}(a',s))$ whenever $\ew\rightarrow0$ (see \cref{proof:convergence_boltzmann}), which is an optimal policy. The simple objective $\argmin(\mathcal{L}(\omega))\coloneqq\argmin(\ew)$ therefore satisfies \circled{1}. Moreover, when our objective is not minimised, we have $\ew>0$ and from \cref{eq:action_posterior} we see that $\piw$ is non-deterministic \textit{for all non-optimal $\omega$}. $\mathcal{L}(\omega)$ therefore satisfies \circled{2} as any agent following $\piw$ will continue exploring until the RL problem is solved. To generalise our framework, we extend $\tw\boldsymbol{\cdot}$ to any operator from the set of target operators $\tw\boldsymbol{\cdot}\in \mathbb{T}$:

\begin{definition}[Target Operator Set]\label{def:target_set}
Define $\mathbb{T}$ to be the set of target operators such that an optimal Bellman operator for $\hQ$ is recovered when the Boltzmann policy in \cref{eq:action_posterior} is greedy with respect to $\hQ$, i.e., $\mathbb{T}\coloneqq\{\tw\boldsymbol{\cdot}\vert\lim_{\ew\rightarrow0}\piw\implies \tw \hQ=\mathcal{T}^*\hQ\}$.
\end{definition}
As an illustration, we prove in \cref{sec:discussion_T} that the Bellman operator $\mathcal{T}^{\pi_\omega}\boldsymbol{\cdot}$ introduced above is a member of $\mathbb{T}$ and can be approximated by several well-known RL targets. We also discuss how $\mathcal{T}^{\pi_\omega}\boldsymbol{\cdot}$ induces a constraint on $\Omega$ due to its recursive definition. As we show in \cref{sec:analysis}, there exists an $\omega$ in the constrained domain that maximises the RL objective under these conditions, so an optimal solution is always feasible. Moreover, we provide an analysis in \cref{sec:analysis_of_approximations} to establish that such a policy is an attractive fixed point for our algorithmic updates, even when we ignore this constraint. Off-policy operators will not constrain $\Omega$: by definition, the optimal Bellman operator $\mathcal{T}^*\boldsymbol{\cdot}$ is a member of $\mathbb{T}$ and does not constrain $\Omega$; similarly, we derive an off-policy operator based on a Boltzmann distribution with a diminishing temperature in \cref{sec:relaxation_constraints} that is a member of  $\mathbb{T}$. Observe that soft Bellman operators are not members of $\mathbb{T}$ as the optimal policy under $J_\text{merl}^\pi$ is not deterministic, hence algorithms such as SAC cannot be derived from the \textsc{virel} framework.

One problem remains: calculating the normalisation constant to sample directly from the Boltzmann distribution in \cref{eq:action_posterior} is intractable for many MDPs and function approximators. As such, we look to variational inference to learn an approximate \textit{variational policy} $\pit\approx\piw$, parametrised by $\theta\in\Theta$ with finite variance and the same support as $\piw$. This suggests optimising a new objective that penalises $\pit$ when $\pit\ne\piw$ but still has a global maximum at $\ew=0$. A tractable objective that meets these requirements is the evidence lower bound (ELBO) on the unnormalised potential of the Boltzmann distribution, defined as $\{\omega^*,\theta^*\}\in\argmax_{\omega,\theta}\mathcal{L}(\omega,\theta)$, \vspace{-0.2cm}
\begin{align}
 \mathcal{L}(\omega,\theta)&\coloneqq\mathbb{E}_{s\sim d(s)}\left[\mathbb{E}_{a\sim \pit} \left[\frac{\hQ}{\ew}\right]+\mathscr{H}(\pit)\right],\label{eq:elborl}
\end{align}
where $\qt\coloneqq d(s)\pit$ is a variational distribution,  $\mathscr{H}(\boldsymbol{\cdot})$ denotes the differential entropy of a distribution, and $d(s)$ is any arbitrary sampling distribution with support over $\mathcal{S}$. From \cref{eq:elborl}, maximising our objective with respect to $\omega$ is achieved when $\ew\rightarrow0$ and hence $\mathcal{L}(\omega,\theta)$  satisfies \circled{1} and \circled{2}. As we show in \cref{proof:objective_infinity}, $\mathscr{H}(\cdot)$ in \cref{eq:elborl} causes $\lp\rightarrow-\infty$ whenever $\pi_\theta(a\vert s)$ is a Dirac-delta distribution for all $\ew>0$. This means our objective heavily penalises premature convergence of our variational policy to greedy Dirac-delta policies except under optimality. We discuss a probabilistic interpretation of our framework in \cref{sec:probablistic_interpretation}, where it can be shown that $\piw$ characterises our model's uncertainty in the optimality of $\hQ$.

We now motivate $\lp$ from an inference perspective: In \cref{sec:derivation_elbo}, we write $\lp$ in terms of the log-normalisation constant of the Boltzmann distribution and the KL divergence between the action-state normalised Boltzmann distribution, $\pw(h)$, and the variational distribution, $\qt$:
\begin{gather}
    \mathcal{L}(\omega,\theta)=\ell(\omega)-\kl{q_\theta(h)}{\pw(h)}-\mathscr{H}(d(s)),\label{eq:objective_ii}\\
    \mathrm{where}\quad\mathcal{\ell}(\omega)\coloneqq\log\int_\mathcal{H}\exp\left(\frac{\hQ}{\ew}\right)dh,\quad \pw(h)\coloneqq \frac{\exp\left(\frac{\hQ}{\ew}\right)}{\int_\mathcal{H}\exp\left(\frac{\hQ}{\ew}\right)dh}.
\end{gather}
As the KL divergence in \cref{eq:objective_ii} is always positive and the final entropy term has no dependence on $\omega$ or $\theta$, maximising our objective for $\theta$ always reduces the KL divergence between $\piw$ and $\pit$ for any $\ew>0$, with $\pit=\piw$ achieved under exact representability (see \cref{proof:policy_posterior}). This yields a tractable way to estimate $\piw$ at any point during our optimisation procedure by maximising $\lp$ for $\theta$. From \cref{eq:objective_ii}, we see that our objective satisfies \circled{3}, as we minimise the mode-seeking direction of KL divergence, $\kl{\qt}{\pw(h)}$, and our objective is an ELBO, which is the starting point for inference algorithms \citep{Jordan1999,Beal03,vi_tutorial}. When the RL problem is solved and $\ew=0$, our objective tends towards infinity for \emph{any} variational distribution that is non-deterministic (see \cref{proof:objective_infinity}). This is of little consequence, however, as whenever $\ew=0$, our approximator is the optimal value function, $\hat{Q}_{\omega^*}(h)=Q^*(h)$ (\cref{proof:forward}), and hence, $\pi^*(a\vert s)$ can be inferred exactly by finding $\max_{a'}\hat{Q}_{\omega^*}(a',s)$ or by using the policy gradient $\nabla_\theta\mathbb{E}_{d(s)\pit}\left[\hat{Q}_{\omega^*}(h)\right]$ (see \cref{sec:ac_discuss}). 
\vspace{-0.6cm}
\subsection{Theoretical Results}
\label{sec:analysis}
\vspace{-0.1cm}
We now formalise the intuition behind \circled{1}-\circled{3}. \cref{proof:convergence_boltzmann} establishes the emergence of a Dirac-delta distribution in the limit of $\ew\rightarrow0$. To the authors' knowledge, this is the first rigorous proof of this result. \cref{proof:forward} shows that finding an optimal policy that maximises the RL objective in \cref{eq:rl_objective} reduces to finding the Boltzmann distribution associated with the parameters $\omega^*\in\argmax_{\omega}\lp$. The existence of such a distribution is a sufficient condition for the policy to be optimal. \cref{proof:policy_posterior} shows that whenever $\ew>0$, maximising our objective for $\theta$ always reduces the KL divergence between $\piw$ and $\pit$, providing a tractable method to infer the current Boltzmann policy. 

\begin{theorem}[Convergence of Boltzmann Distribution to Dirac Delta]\label{proof:convergence_boltzmann}
Let $p_\varepsilon:\mathcal{X}\rightarrow[0,1]$ be a Boltzmann distribution with temperature $\varepsilon\in\mathbb{R}_{\ge0}$, $p_\varepsilon(x)=\frac{\exp\left(\frac{f(x)}{\varepsilon}\right)}{\int_\mathcal{X}\exp\left(\frac{f(x)}{\varepsilon}\right)dx},$ where $f:\mathcal{X}\rightarrow\mathcal{Y}$ is a function that satisfies \cref{def:locally_smooth}. In the limit $\varepsilon\rightarrow 0$, $p_\varepsilon(x)\rightarrow \delta(x=\sup_{x'} f(x'))$.
\begin{proof}
\vspace{-0.4cm}
See \cref{sec:convergence_boltzmann}
\vspace{-0.2cm}
\end{proof}
\end{theorem}
\begin{lemma}[Lower and Upper limits of $\lp$] i) For any $\ew>0$ and $\pit=\delta(a^*)$, we have $\lp=-\infty$. ii) For $\hQ>0$ and any non-deterministic $\pit$, $\lim_{\ew\rightarrow0}\lp=\infty$.
\label{proof:objective_infinity}
\begin{proof}
\vspace{-0.4cm}
See \cref{proof:rl_elbo_ap}.
\vspace{-0.2cm}
\end{proof}
\end{lemma}

\begin{theorem}[Optimal Boltzmann Distributions as Optimal Policies]
	\label{proof:forward}
	For $\omega^*$ that maximises $\lp$ defined in \cref{eq:elborl}, the corresponding Boltzmann policy induced must be optimal, i.e., $\{\omega^*,\theta^*\} \in \argmax_{\omega,\theta}\lp
	\implies  \pi_{\omega^*}(a \vert  s) \in \Pi^*$.
\begin{proof}
\vspace{-0.4cm}
See \cref{proof:rl_elbo_ap}.
\vspace{-0.2cm}
\end{proof}
\end{theorem}
\begin{theorem}[Maximising the ELBO for $\theta$]
\label{proof:policy_posterior}
 For any $\ew>0$, $\max_\theta\lp=\mathbb{E}_{d(s)}\left[\min_\theta\kl{\pit}{\piw}\right]$ with $\piw=\pit$ under exact representability. 
\begin{proof}
\vspace{-0.4cm}
See \cref{sec:proof_kl_app}.
\vspace{-0.2cm}
\end{proof}
\end{theorem}

\subsection{Comparing \textsc{virel} and \textsc{merlin} Frameworks} 
\label{sec:comparing_virel_merlin}
 \begin{wrapfigure}{r}{0.42\textwidth}
\vspace{-1.6cm}
    \begin{center}
    \includegraphics[scale=0.167]{rl_vinference.png}
    \end{center}
  \caption{Graphical models for \textsc{merlin} and \textsc{virel} (variational approximations are dashed).}
  \label{fig:rl_vi_graphs}
  \vspace{-0.5cm}
\end{wrapfigure}

To compare \textsc{merlin} and \textsc{virel}, we consider the probabilistic interpretation of the two models discussed in \cref{sec:probablistic_interpretation}; introducing a binary variable $\mathcal{O}\in\{0,1\}$ defines a graphical model for our inference problem whenever $\ew>0$. Comparing the graphs in \cref{fig:rl_vi_graphs}, observe that \textsc{merlin} models exponential \emph{cumulative} rewards over entire trajectories. By contrast, \textsc{virel}'s variational policy models a single step and a function approximator is used to model future \emph{expected} rewards. The resulting KL divergence minimisation for \textsc{merlin} is therefore much more sensitive to the value of temperature, as this affects how much future entropy influences the variational policy. For \textsc{virel}, temperature is defined by the model, and updates to the variational policy will not be as sensitive to errors in its value or linear scaling as its influence only extends to a single interaction. We hypothesise that \textsc{virel} may afford advantages in higher dimensional domains where there is greater chance of encountering large regions of state-action space with sub-optimal reward; like our counterexample from \cref{sec:background}, $c$ must be comparatively small to balance the influence of entropy in these regions to prevent $\textsc{merlin}$ algorithms from learning sub-optimal policies.

\cref{proof:convergence_boltzmann} demonstrates that, unlike in \textsc{merlin}, \textsc{virel} naturally learns optimal deterministic policies directly from the optimisation procedure while still maintaining the benefits of stochastic policies in training. While Boltzmann policies with fixed temperatures have been proposed before \citep{Sallans04}, the adaptive temperature $\ew$ in \textsc{virel}'s Boltzmann policy is unique in that it ensures adaptive exploration that becomes less stochastic as $\hQ\rightarrow Q^*(h)$. Like in \textsc{merlin}, we discuss a probabilistic interpretation of this policy as a posterior over actions conditioned on $\mathcal{O}=1$ in \cref{sec:probablistic_interpretation}.

==> VIREL NeurIPS i/sections/related.tex <==
 



==> sections/related.tex <==
 


